Adaptive Coding and Channel Shaping Through Reconfigurable Intelligent Surfaces: An Information-Theoretic Analysis

A communication link aided by a reconfigurable intelligent surface (RIS) is studied in which the transmitter can control the state of the RIS via a finite-rate control link. Channel state information (CSI) is acquired at the receiver based on pilot-assisted channel estimation, and it may or may not be shared with the transmitter. Considering quasi-static fading channels with imperfect CSI, capacity-achieving signalling is shown to implement joint encoding of the transmitted signal and of the response of the RIS. This demonstrates the information-theoretic optimality of RIS-based modulation, or "single-RF MIMO" systems. In addition, a novel signalling strategy based on separate layered encoding that enables practical successive cancellation-type decoding at the receiver is proposed. Numerical experiments show that the conventional scheme that fixes the reflection pattern of the RIS, irrespective of the transmitted information, as to maximize the achievable rate is strictly suboptimal, and is outperformed by the proposed adaptive coding strategies at all practical signal-to-noise ratio (SNR) levels.

==> packages_commands_theorems.tex <==

\usepackage[utf8]{inputenc} 


\usepackage[T1]{fontenc}


\usepackage{cite}


\ifCLASSINFOpdf
 \usepackage[pdftex]{graphicx}
 \graphicspath{{../pdf/}{../jpeg/}}
 \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\else
 \usepackage[dvips]{graphicx}
 \graphicspath{{../eps/}}
 \DeclareGraphicsExtensions{.eps}
\fi



\usepackage[cmex10]{amsmath}  
\DeclareMathOperator*{\argmax}{arg\,max} 
\DeclareMathOperator*{\argmin}{arg\,min} 
\usepackage{amssymb}
\interdisplaylinepenalty=2500 


\usepackage{algorithmic}


\usepackage{array}


\usepackage{stfloats}

\usepackage{flafter}


\usepackage{url}


\usepackage{cases}

\usepackage[colorlinks = true]{hyperref}


\usepackage{tikz}
\usetikzlibrary{calc} 
\usepackage{pgfplots}
\usetikzlibrary{patterns}
\usetikzlibrary{positioning}
\usetikzlibrary{arrows.meta} 
\usetikzlibrary{shapes} 
\usetikzlibrary{shapes.geometric} 
\usetikzlibrary{fit} 



\RequirePackage{microtype}


\usepackage{xcolor}
\definecolor{TechnionBlue}{rgb}{0, 0.1765, 0.3843} 
\definecolor{OliveGreen}{rgb}{0.4, 0.62, 0.25} 


\usepackage{ifthen}



\usepackage[normalem]{ulem}


\usepackage{fontawesome}



\newcommand{\rb}[1] {\left(#1\right)}
\newcommand{\cb}[1] {\left\lbrace #1 \right\rbrace}
\newcommand{\sqb}[1] {\left[#1\right]}
\newcommand{\given}[1]{\left\lvert#1\right.}
\newcommand{\AgivenB}[2]{\left(#1\middle\vert#2\right)}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand*{\QEDA}{\hfill\ensuremath{\blacksquare}}
\newcommand*{\nspace}[1] {
	\ifthenelse{\equal{#1}{!}}{\!}{} 
	\ifthenelse{\equal{#1}{tq}}{\kern-1em}{} 
	\ifthenelse{\equal{#1}{mq}}{\mkern-18mu}{} 
}



\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}



\DeclareMathOperator{\tr}{tr}


